Absorption time and absorption probabilities for a family of multidimensional gambler models

For a family of multidimensional gambler models we provide formulas for the winning probabilities (in terms of parameters of the system) and for the distribution of game duration (in terms of eigenvalues of underlying one-dimensional games). These formulas were known for one-dimensional case - initially proofs were purely analytical, later probabilistic construction has been given. Concerning the game duration, in many cases our approach yields sample-path constructions. We heavily exploit intertwining between (not necessary) stochastic matrices (for game duration results), a notion of Siegmund duality (for winning/ruin probabilities), and a notion of Kronecker products.

==> sections/ehrenfest.tex <==
Let $X^*$ be a Markov Chain on the state space $ \E=\{1\ldots d\}$ with transition matrix ${\PP}_{X^*}$ of the form:
 $$
 {\PP}_{X^*}(i,i')=\left\{
 \begin{array}{llll}  
  \frac{d-i}{2d-2}\frac{\sum_{r=0}^{i-1} {{d-1} \choose {r-1}} }{\sum_{r=0}^{i} {{d-1} \choose {r-1}}}  & \mathrm{if }\  i'=i-1, i<d \\
  \frac{d-2}{2d-2} & \mathrm{if} \ i'=i, i < d, \\
  1 & \mathrm{if} \ i'=i= d, \\
   \frac{i}{2d-2}\frac{\sum_{r=0}^{i+1} {{d-1} \choose {r-1}} }{\sum_{r=0}^{i} {{d-1} \choose {r-1}}}   & \mathrm{if }\  i'=i+1, \\
  0 & \mathrm{otherwise}, \\
 \end{array}\right.
 $$
and initial distribution $\nu^*(j)=\mathbbm{1}_{j=m}$, e.g. $X^*$ starts in the state $m$. Then the time to absorption in this chain has pgf of the form:

$$ pgf_{T_{\nu^*,d}^*}(s)=
\sum_{j\in {\E}} \hat{\nu}(j) pgf_{\hat{T}_{j,d}}(s),$$
where:

 $$ \hat{\nu}(j) = \frac{2^{j-1}(-1)^{i+j}(i-j+1){{d-1}\choose{i}}{{i}\choose{j-1}}}{(d-j)\sum_{m=0}^{i-1}{{d-1}\choose{m}}},$$
and:
$$pgf_{\hat{T}_{j,d}}(s)=\prod_{k=j}^{d-1} \left[{(1-\frac{k-1}{d-1})s\over 1-\frac{k-1}{d-1} s}\right].$$

\begin{proof}
Let us define $\Lambda$ :
 $$ \Lambda(i,j)=\left\{
 \begin{array}{llll} 
 \frac{(i-1)!(d-j)!(d-i)\sum_{k=0}^{j-1}{{d-1}\choose{k}}}{(d-1)!(i-j)!(d-j)2^{i-1}} & \mathrm{if} \ j\leq i<d, \\ 
  0 & i<j\leq d, \\
  1 & j=d, i =d. \\
 \end{array}\right.
 $$
 Then:
   $$ \Lambda^{-1}(i,j)=\left\{
 \begin{array}{llll}  
  \frac{2^{j-1}(-1)^{i+j}(i-j+1){{d-1}\choose{i}}{{i}\choose{j-1}}}{(d-j)\sum_{m=0}^{i-1}{{d-1}\choose{m}}} & \mathrm{if} \ j<d, \\
  0 & j=d, i<d \\
  1 & j=d, i =d. \\
 \end{array}\right.
 $$ 
 Let:
  $$
 {\PP}_{\hat{X}}(i,i')=\left\{
 \begin{array}{llll}  
  \frac{i-1}{d-1} & \mathrm{if} \ i'=i, \\
  \frac{d-i}{d-1}  & \mathrm{if }\  i'=i+1, \\
  0 & \mathrm{otherwise}. \\
 \end{array}\right.
 $$

Now we can check that $\Lambda\PP_{X^*}=\PP_{\hat{X}}\Lambda$.

Case $i=d,j=d$:

$$\Lambda\PP_{X^*}(d,d)=\Lambda(d,d)\PP_{X^*}(d,d)=1*1=1$$
$$\PP_{\hat{X}}\Lambda(d,d)=\PP_{\hat{X}}(d,d)\Lambda(d,d)=1*1=1$$

Case $i=d,j<d$:

$$\Lambda\PP_{X^*}(d,j)=0$$
$$\PP_{\hat{X}}\Lambda(d,j)=0$$

Case $j\geq i+1$:

$$\Lambda\PP_{X^*}(i,i+1)=\Lambda(i,i)\PP_{X^*}(i,i+1)=\frac{(i-1)!(d-i)!(d-i)\left(\sum_{k=0}^{i-1}{{d-1} \choose {k}}\right) i\left( \sum_{k=0}^{i+1} {{d-1}\choose{k-1}} \right)}{(d-1)!(i-i)!(d-i)2^{i-1} 2(d-1) \left(\sum_{k=0}^{i} {{d-1}\choose{k-1}} \right)}$$

$$\PP_{\hat{X}}\Lambda(i,i+1)=\frac{i!(d-i-1)!(d-i-1)\left( \sum_{k=0}^i {{d-1}\choose {k} } \right) (d-i) }{(d-1)!(i+1-i-1)!(d-i-1)2^i (d-1)}$$

Case $j=i<d$:

$$\Lambda\PP_{X^*}(i,i)=\Lambda(i,i-1)\PP_{X^*}(i-1,i)+\Lambda(i,i)\PP_{X^*}(i,i)$$
$$=\Lambda(i,i-1)\PP_{X^*}(i-1,i)+\Lambda(i,i)\PP_{X^*}(i,i)$$
$$=\frac{(i-1)!(d-i+1)!(d-i)\left(\sum_{k=0}^{i-2}{{d-1} \choose {k}}\right) (i-1)\left( \sum_{k=0}^{i} {{d-1}\choose{k-1}} \right)}{(d-1)!(i-i+1)!(d-i+1)2^{i-1} 2(d-1) \left(\sum_{k=0}^{i-1} {{d-1}\choose{k-1}} \right)}+$$
$$+\frac{(i-1)!(d-i)!(d-i)\left(\sum_{k=0}^{i-1}{{d-1} \choose {k}}\right) (d-2)}{(d-1)!(i-i)!(d-i)2^{i-1} 2(d-1) }$$

$$\PP_{\hat{X}}\Lambda(i,i)=\PP_{\hat{X}}(i,i+1)\Lambda(i+1,i)+\PP_{\hat{X}}(i,i)\Lambda(i,i)$$
$$=\frac{i!(d-i)!(d-i-1)\left( \sum_{k=0}^{i-1} {{d-1}\choose {k} } \right) (d-i) }{(d-1)!(i+1-i)!(d-i)2^i (d-1)}+$$
$$+\frac{(i-1)!(d-i)!(d-i)\left( \sum_{k=0}^{i-1} {{d-1}\choose {k} } \right) (i-1) }{(d-1)!(i-i)!(d-i)2^{i-1} (d-1)}$$

Case $j<i<d$:

$$\Lambda\PP_{X^*}(i,j)=\Lambda(i,j-1)\PP_{X^*}(j-1,j)+\Lambda(i,j)\PP_{X^*}(j,j)+\Lambda(i,j+1)\PP_{X^*}(j+1,j)$$
$$=\frac{(i-1)!(d-j+1)!(d-i)\sum_{k=0}^{j-2}{{d-1}\choose{k}} (j-1)  \sum_{k=0}^{j}{{d-1}\choose{k-1}}} { (d-1)!(i-j+1)!(d-j+1)2^{i-1} 2(d-1) \sum_{k=0}^{j-1}{{d-1}\choose{k-1}}  } +$$
$$+\frac{(i-1)!(d-j)!(d-i)\sum_{k=0}^{j-1}{{d-1}\choose{k}} (d-2)  } { (d-1)!(i-j)!(d-j)2^{i-1} 2(d-1)} $$
$$=\frac{(i-1)!(d-j-1)!(d-i)\sum_{k=0}^{j}{{d-1}\choose{k}} (d-j-1)  \sum_{k=0}^{j}{{d-1}\choose{k-1}}} { (d-1)!(i-j-1)!(d-j-1)2^{i-1} 2(d-1) \sum_{k=0}^{j+1}{{d-1}\choose{k-1}}  } +$$

$$\PP_{\hat{X}}\Lambda(i,i)=\PP_{\hat{X}}(i,i)\Lambda(i,j)+\PP_{\hat{X}}(i,i+1)\Lambda(i+1,j)$$
$$=\frac{(i-1)!(d-j)!(d-i)\left( \sum_{k=0}^{j-1} {{d-1}\choose {k} } \right) (i-1) }{(d-1)!(i-j)!(d-j)2^{i-1} (d-1)}+$$
$$+\frac{i!(d-j)!(d-i-1)\left( \sum_{k=0}^{j-1} {{d-1}\choose {k} } \right) (d-i) }{(d-1)!(i-j+1)!(d-j)2^i (d-1)}$$

So assumptions of (\ref{lem:duality_two_linksC}) are fulfilled for $\hat{\nu}=\nu^*\Lambda^{-1}$.
 Then we have 

$$pgf_{T^*_{\nu^*,\e_M^*}}(s) = \Lambda(\hat{\e}_M,\e_M^*)  \sum_{\hat{\e}\in \hat{\E}} \hat{\nu}(\hat{\e}) pgf_{\hat{T}_{\hat{\e},\hat{\e}_M}}(s),$$
where $\Lambda(\hat{\e}_M,\e_M^*)=1$,  $ \hat{\nu}(j) = \nu^*\Lambda^{-1}=\frac{2^{j-1}(-1)^{i+j}(i-j+1){{d-1}\choose{i}}{{i}\choose{j-1}}}{(d-j)\sum_{m=0}^{i-1}{{d-1}\choose{m}}},$ and $pgf_{\hat{T}_{j,d}}(s)$ is a probability generating function of pure-birth Markov chain which was analyzed in (\ref{eq:gT1}).
\end{proof}
\begin{proof}
expectation:
$$pgf_{\hat{T}_{j,d}}'(1)=(d-1)\sum_{k=j}^{d-1} \frac{1}{d-k}$$
\end{proof}

Taking $\PP$ a Markov Chain transition matrix of Ehrenfest model with $N$ states we can consider its SSD Dual $\PP^*$. It was calculated in ... that the link $\Lambda^*$ ($\PP=(\Lambda^*)^{-1}\PP^*\Lambda^*$) between those two matrices have truncated binomial distribution in each row. On the other hand we know from ... that spectral dual $\hat{\PP}$ ($\PP=(\hat{\Lambda})^{-1}\hat{\PP}\hat{\Lambda}$) of Ehrenfest transition matrix have its eigenvalues (k/n) on the diagonal - so we know its pgf. Compiling those two observations we can conclude that the pgf of $\PP^*$ is the same as $\hat{\PP}$ with proper $\Lambda=\Lambda^*\hat{\Lambda}^{-1}$.

...dokładniej

dim=d



% ssd dual - recurrence def, for $xi(n,m)=X(n,m)=(n-m+1)m$: \url{https://oeis.org/A003991} :
% $$
% {\PP}_{X^*}(i,i')=\left\{
% \begin{array}{llll}  
%  \frac{\xi(d-2,i-1)}{4(d-1)^2 p_{i-1}}  & \mathrm{if }\  i'=i-1, \\
%  \frac{d-2}{2d-2} & \mathrm{if} \ i'=i, i \neq d, \\
%  1 & \mathrm{if} \ i'=i= d, \\
%  1-q_i-r  & \mathrm{if }\  i'=i+1, \\
%  0 & \mathrm{otherwise}. \\
% \end{array}\right.
% $$
%$ \xi(d-2,i-1)=(d-i)(i-1)$
%
%$q_i={\PP}_{X^*}(i,i-1)$
%
%$p_i={\PP}_{X^*}(i,i+1)$
% 

ssd dual:
%można zapisać przy pomocy funkcji hipergeometrycznej
 $$
 {\PP}_{X^*}(i,i')=\left\{
 \begin{array}{llll}  
  \left( \frac{1}{2}-\frac{i-1}{2d-2}\right)\frac{\sum_{r=0}^{i-1} {{d-1} \choose {r-1}} }{\sum_{r=0}^{i} {{d-1} \choose {r-1}}}  & \mathrm{if }\  i'=i-1, i<d \\
  \frac{d-2}{2d-2} & \mathrm{if} \ i'=i, i < d, \\
  1 & \mathrm{if} \ i'=i= d, \\
  \left( \frac{1}{2}-\frac{d-i-1}{2d-2}\right)\frac{\sum_{r=0}^{i+1} {{d-1} \choose {r-1}} }{\sum_{r=0}^{i} {{d-1} \choose {r-1}}}   & \mathrm{if }\  i'=i+1, \\
  0 & \mathrm{otherwise}. \\
 \end{array}\right.
 $$
 
Ehrenfest:
$$
 {\PP}_{X}(i,i')=\left\{
 \begin{array}{llll}  
   \frac{i-1}{2(d-1)} & \mathrm{if }\  i'=i-1, \\
  1/2 & \mathrm{if} \ i'=i, \\
  \frac{d-i}{2(d-1)}  & \mathrm{if }\  i'=i+1, \\
  0 & \mathrm{otherwise}. \\
 \end{array}\right.
 $$
 
 spectral:
 $$
 {\PP}_{\hat{X}}(i,i')=\left\{
 \begin{array}{llll}  
  \frac{i-1}{d-1} & \mathrm{if} \ i'=i, \\
  \frac{d-i}{d-1}  & \mathrm{if }\  i'=i+1, \\
  0 & \mathrm{otherwise}. \\
 \end{array}\right.
 $$
 Lambda SSD:
 $$ \Lambda^*(i,j)=\frac{{{d-1}\choose{j-1}}}{\sum_{k=0}^{i-1}{{d-1}\choose{k}}}\mathbbm{1}_{0\leq j \leq i}$$
 Lambda SSD \^ -1 (nieistotna, ale tutaj: 
\begin{verbatim}
\url{https://oeis.org/search?q=1%2C5%2C11%2C15%2C16&sort=&language=polish&go=Wyszukaj)} : 
\end{verbatim}

  $$ (\Lambda^*)^{-1}(i,i')=\left\{
 \begin{array}{llll}  
  -\frac{\sum_{k=0}^{i-2}{{d-1}\choose{k}} }{{{d-1}\choose{i-1}}} & \mathrm{if} \ i'=i-1, \\
  \frac{\sum_{k=0}^{i-1}{{d-1}\choose{k}}}{{{d-1}\choose{i-1}}}  & \mathrm{if }\  i'=i, \\
  0 & \mathrm{otherwise}. \\
 \end{array}\right.
 $$
 Lambda spectral:
  $$ \hat{\Lambda}(i,j)=\frac{{{i-1}\choose{j-1}}}{2^{i-1}}$$
  
  Lambda spectral \^ -1 ,tutaj: 
  \begin{verbatim}
 \url{https://oeis.org/search?q=1%2C+-8%2C+24%2C+-32%2C+16&language=english&go=Search} :
 \end{verbatim}
  $$ \hat{\Lambda}^{-1}(i,j)=(-1)^{j-i}2^{j-1}{{i-1}\choose{j-1}}$$
  Lambda $\Lambda=\Lambda^*\hat{\Lambda}^{-1}$ :
   $$ \Lambda(i,j)=\left\{
 \begin{array}{llll}  
  \frac{2^{j-1}(-1)^{i+j}(i-j+1){{d-1}\choose{i}}{{i}\choose{j-1}}}{(d-j)\sum_{m=0}^{i-1}{{d-1}\choose{m}}} & \mathrm{if} \ j<d, \\
  0 & i=d, j<d \\
  1 & j=d, i =d. \\
 \end{array}\right.
 $$
  Lambda -1:
  $$ \Lambda^{-1}(i,j)=\left\{
 \begin{array}{llll} 
 \frac{(i-1)!(d-j)!(d-i)\sum_{k=0}^{j-1}{{d-1}\choose{k}}}{(d-1)!(i-j)!(d-j)2^{i-1}} & \mathrm{if} \ j\leq i<d, \\ 
  0 & i<j\leq d \\
  1 & j=d, i =d. \\
 \end{array}\right.
 $$
 
  For (i-ustalone) $\nu(j)=\mathbbm{1}_{j=i}$ :
  $$ \hat{\nu}(j) = \frac{2^{j-1}(-1)^{i+j}(i-j+1){{d-1}\choose{i}}{{i}\choose{j-1}}}{(d-j)\sum_{m=0}^{i-1}{{d-1}\choose{m}}}$$
"proof":
$$ \hat{\nu}(j)=(\nu\Lambda^*\hat{\Lambda}^{-1})(j)=\sum_{j\leq k \leq i}\Lambda^*(i,k)\hat{\Lambda}^{-1}(k,j)$$
$$=\sum_{j\leq k \leq i}\frac{{{d-1}\choose{k-1}}}{\sum_{m=0}^{i-1}{{d-1}\choose{m}}}\mathbbm{1}_{0\leq k \leq i}(-1)^{j+k}2^{j-1}{{k-1}\choose{j-1}}$$  
  $$=\frac{2^{j-1}}{\sum_{m=0}^{i-1}{{d-1}\choose{m}}}\sum_{j\leq k \leq i}(-1)^{j+k}{{d-1}\choose{k-1}}{{k-1}\choose{j-1}}$$ 
  
wiki: 
\begin{verbatim}
 \url{https://en.wikipedia.org/wiki/Binomial_coefficient}
\end{verbatim}

(1)

$\sum_{j=0}^{k}(-1)^j{{n}\choose{j}}=(-1)^k{{n-1}\choose{k}}$ so (for j->k,k->i-j,n->d-j) $\sum_{k=0}^{i-j}(-1)^k{{d-j}\choose{k}}=(-1)^{i-j}{{d-j-1}\choose{i-j}}$

and 

(2)

${{d-1}\choose{k-1}}{{k-1}\choose{j-1}}={{d-1}\choose{j-1}}{{d-j}\choose{d-k}}$

from (2)

$$=\frac{2^{j-1}}{\sum_{m=0}^{i-1}{{d-1}\choose{m}}}\sum_{j\leq k \leq i}(-1)^{j+k}{{d-1}\choose{j-1}}{{d-j}\choose{d-k}}$$ 


$$=\frac{2^{j-1}}{\sum_{m=0}^{i-1}{{d-1}\choose{m}}}{{d-1}\choose{j-1}}\sum_{j\leq k \leq i}(-1)^{j+k}{{d-j}\choose{d-k}}$$ 
$$=\frac{2^{j-1}}{\sum_{m=0}^{i-1}{{d-1}\choose{m}}}{{d-1}\choose{j-1}}\sum_{j\leq k \leq i}(-1)^{j+k}{{d-j}\choose{k-j}}$$ 
$$=\frac{2^{j-1}}{\sum_{m=0}^{i-1}{{d-1}\choose{m}}}{{d-1}\choose{j-1}}\sum_{k=0}^{i-j}(-1)^{2j+k}{{d-j}\choose{k}}$$ 
$$=\frac{2^{j-1}}{\sum_{m=0}^{i-1}{{d-1}\choose{m}}}{{d-1}\choose{j-1}}\sum_{k=0}^{i-j}(-1)^{k}{{d-j}\choose{k}}$$ 

from (1)
$$=\frac{2^{j-1}}{\sum_{m=0}^{i-1}{{d-1}\choose{m}}}{{d-1}\choose{j-1}}(-1)^{i-j}{{d-j-1}\choose{i-j}}$$ 

\textcolor{green}{
$$=\frac{2^{j-1}(-1)^{i+j}}{\sum_{m=0}^{i-1}{{d-1}\choose{m}}}\frac{(d-1)!(d-j-1)!i!}{(j-1)!(d-j)!(i-j)!(d-i-1)!i!}$$ 
$$=\frac{2^{j-1}(-1)^{i+j}}{\sum_{m=0}^{i-1}{{d-1}\choose{m}}}\frac{(d-1)!i!(i-j+1)}{i!(d-i-1)!(j-1)!(i-j+1)!(d-j)}$$ 
$$=\frac{2^{j-1}(-1)^{i+j}(i-j+1)}{(d-j)\sum_{m=0}^{i-1}{{d-1}\choose{m}}} {{d-1}\choose{i}}{{i}\choose{j-1}}$$ 
}


==> sections/ehrenfest2_old.tex <==

Here we present a concrete example of a birth and death chain on $\E=\{1,\ldots,N\}$ with $N$ being
the only absorbing state, for which we provide $pgf$ of absorption time provided chain started at any $m\in \E$.
We use Lemma \ref{lem:duality_two_linksC} calculating link $\Lambda$. As far as we are aware, this $pgf$ 
cannot be given using results from \cite{Gong2012} \ie (\ref{eq:gTi}). 
This is since the eigenvalues the presented matrix $\PP_{X^*}$ are known, 
but the eigenvalues of $ \PP_{Y}^{\ceil{m}}$ are not known for any $m\in\E$.
\medskip\par 

\textcolor{red}{zmienilem $d$ na $N$ ... bo bylo mylace - wczesniej $d$ oznaczalo wymiar...
}

\textcolor{green}{ok}

\begin{example}  
Let $X^*$ be a Markov Chain on the state space $ \E=\{1,\ldots, N\}$ with transition matrix ${\PP}_{X^*}$ of the form:
 $$
 {\PP}_{X^*}(i,i')=\left\{
 \begin{array}{llll}  
  \frac{N-i}{2N-2}\frac{\sum_{r=0}^{i-1} {{N-1} \choose {r-1}} }{\sum_{r=0}^{i} {{N-1} \choose {r-1}}}  & \mathrm{if }\  i'=i-1, i<N \\[12pt]
  \frac{N-2}{2N-2} & \mathrm{if} \ i'=i, i < N, \\[12pt]
  1 & \mathrm{if} \ i'=i= N, \\[12pt]
   \frac{i}{2N-2}\frac{\sum_{r=0}^{i+1} {{N-1} \choose {r-1}} }{\sum_{r=0}^{i} {{N-1} \choose {r-1}}}   & \mathrm{if }\  i'=i+1, \\[12pt]
  0 & \mathrm{otherwise}, \\
 \end{array}\right.
 $$
%and initial distribution $\nu^*(j)=\mathbb{1}_{j=m}$, e.g. $X^*$ starts in the state $m$.
Then the absorption time starting at $m\in\E $ is has the following $pgf$:

\textcolor{red}{zmienilem sumowanie z ${j\in {\E}}$ na $j\leq m$, zamiast $T^*_{\nu^*,d}$ pisze $T^*_{m,d}$}

\textcolor{green}{ok}
 \begin{equation}\label{eq:ex_c_pgf}
 pgf_{T_{m,d}^*}(s)=\sum_{j\leq m} \hat{\nu}(j) pgf_{\hat{T}_{j,d}}(s),
\end{equation}
where (\textcolor{red}{uwaga: zmienilem $i$ na $m$ i sumuje po $k$})

\textcolor{green}{ok}
\begin{equation}\label{eq:hat_mu}
  \hat{\nu}(j) = \frac{2^{j-1}(-1)^{m+j}(m-j+1){{N-1}\choose{m}}{{m}\choose{j-1}}}{(N-j)\sum_{k=0}^{m-1}{{N-1}\choose{k}}}
 \quad and \quad 
 pgf_{\hat{T}_{j,N}}(s)=\prod_{k=j}^{N-1} \left[{(1-\frac{k-1}{N-1})s\over 1-\frac{k-1}{N-1} s}\right].
\end{equation}
 In particular, we have 
 \begin{equation}\label{eq:ex_c_ex}
E(T^*_{m,N})=(N-1)\sum_{j\leq m} \hat{\nu}(j) \sum_{k=j}^{N-1}{1\over N-k}.
\end{equation}

\end{example}
\begin{proof}
Let 
  $$
 {\PP}_{\hat{X}}(i,i')=\left\{
 \begin{array}{llll}  
  \frac{i-1}{N-1} & \mathrm{if} \ i'=i, \\[9pt]
  \frac{N-i}{N-1}  & \mathrm{if }\  i'=i+1, \\[9pt]
  0 & \mathrm{otherwise}. \\
 \end{array}\right.
 $$
 Note that $pgf_{\hat{T}_{j,N}}$ is obviously of form given in (\ref{eq:hat_mu}).
To show the result via Lemma \ref{lem:duality_two_linksC} it is enough 
to find $\Lambda$ such that $\Lambda \PP_{X^*}=\PP_{\hat{X}}\Lambda$ and $\nu^*\Lambda^{-1}=\hat{\nu},$
where $\nu^*(j)=\mathbf{1}(j=m)$.
\par 
However, since $X^*$ has only one absorbing state, we can -- and we will -- follow the \textsl{outline of an alternative proof} 
given in Section \ref{sec:alt}. \textsl{I.e.,} we will indicate intermediate ergodic chain $X$  on $\E$ 
with transition matrix $\PP_X$ and find $\Lambda^*$ and $\hat{\Lambda}$ such that $\Lambda^*\PP_X=\PP_{X^*}\Lambda^*$
and $\hat{\Lambda}\PP_X=\PP_{\hat{X}}\hat{\Lambda}$. Then, we will automatically have 
$\Lambda=\hat{\Lambda} (\Lambda^*)^{-1}$ and we will show that $\nu^*\Lambda^{-1}=\Lambda^*(\hat{\Lambda})^{-1}=\hat{\nu}$.
\medskip\par 
\noindent
Let $X$ be a chain on $\E$ with the following transition matrix: 
$$
 {\PP}_{X}(i,i')=\left\{
 \begin{array}{llll}  
   \frac{i-1}{2(N-1)} & \mathrm{if }\  i'=i-1, \\[9pt]
  {1\over 2} & \mathrm{if} \ i'=i, \\[9pt]
  \frac{N-i}{2(N-1)}  & \mathrm{if }\  i'=i+1, \\[9pt]
  0 & \mathrm{otherwise}, \\
 \end{array}\right.
 $$
 \ie $X$ corresponds to Ehrenfest model of $N$ particles.
 Its stationary distribution is a binomial distribution $\pi(j)={1\over 2^N}{N-1 \choose j-1}$ 
 (we have states enumerated $1,\ldots,N$ what corresponds to $0,\ldots,N-1$ in classical
 Ehrenfest model formulation, \textcolor{green}{i.e. with probability of $\frac{1}{2}$ of staying at the present state}), thus the classical link (cf.  (\ref{eq:link_classic})) is given by 
 $$ \Lambda^*(i,j)=\frac{{{N-1}\choose{j-1}}}{\sum_{k=0}^{i-1}{{N-1}\choose{k}}}\mathbf{1}({ j \leq i}),$$
 \ie we have  $\Lambda^*\PP_X=\PP_{X^*}\Lambda$ ($X^*$ is a sharp SSD of $X$). 
   It can be checked that \textcolor{red}{(pisales, ze nie jest istotna, ale to ta jest istotna, tak?) \textcolor{green}{zrobić sprawdzenie?}}
   $$ (\Lambda^*)^{-1}(i,i')=\left\{
 \begin{array}{llll}  
  -\frac{\sum_{k=0}^{i-2}{{N-1}\choose{k}} }{{{N-1}\choose{i-1}}} & \mathrm{if} \ i'=i-1, \\[12pt]
  \frac{\sum_{k=0}^{i-1}{{N-1}\choose{k}}}{{{N-1}\choose{i-1}}}  & \mathrm{if }\  i'=i, \\[10pt]
  0 & \mathrm{otherwise}. \\
 \end{array}\right.
 $$
 \par 
 \noindent
 The eigenvalues of (Ehrenfest chain) $X$ are known, these are ${i\over N-1}, i=0,\ldots,N-1$,
 \textcolor{red}{czy to jest ok????} \textcolor{green}{teraz tak - zaczynają się od 0 a nie od 1}
 thus $\hat{X}$ is its pure birth spectral dual. The link $\hat{\Lambda}$ such that  $\hat{\Lambda}\PP_X
 =\PP_{\hat{X}}\hat{\Lambda}$ is known
 (see Eq. (4.6) in \cite{Fill2009}), it is given by
 $$\hat{\Lambda}(i,j)={ {i-1\choose j-1}\over 2^{i-1}}.$$
%  It can be checked that 
%   $$ \hat{\Lambda}^{-1}(i,j)=(-1)^{j-i}2^{j-1}{{i-1}\choose{j-1}}.$$
%  
\noindent
Thus, as outlined in Section \ref{sec:alt} we have $\Lambda \PP_{X^*}=\PP_{\hat{X}}\Lambda$ 
 with $\Lambda=\Lambda^*(\hat{\Lambda})^{-1}$ (note that we do not need to calculate it actually) \textcolor{green}{(ale jednak musimy, bo to te same obliczenia co do $\nu^*$, więc chyba można ominąć ten nawias i ostatni Remark przeformułować tak, żeby to był wniosek z obliczenia $\nu^*$)}. We need only to check that $\nu^*\Lambda^{-1}=\nu^*\hat{\Lambda}(\Lambda^*)^{-1}$
 is equal to $\hat{\nu}$ given in (\ref{eq:hat_mu}).
 We have 
 $$(\nu^*\hat{\Lambda}(\Lambda^*)^{-1})(j) = \sum_{k} \hat{\Lambda}(m,k)(\Lambda^*)^{-1}(k,j)$$
 \textcolor{red}{TO DO: pokazac, ze wychodzi to co ma wyjsc, tj. $\hat{\nu}(j)$ dane w  (\ref{eq:hat_mu})}
 \textcolor{green}{zrobiłem to wcześniej - na samym końcu notatek - dodałem dzisiaj jeszcze dwie linijki, żeby było jaśniej - można przenieść te obliczenia tutaj}
 
 Note that $pgf$ given in (\ref{eq:hat_mu}) corresponds to the distribution of $\sum_{k=j}^{N-1} Y_k$, where $Y_k$ is a geometric random variable with parameter ${k-1\over N-1}$ and $Y_1,\ldots,Y_{N-1}$ are independent.
 We have $EY_k={N-1\over N-k}$ thus (\ref{eq:ex_c_ex}) follows from (\ref{eq:ex_c_pgf}) and (\ref{eq:hat_mu}).
 
 \end{proof}
 
 \begin{remark}
  Note that we could  calculate $\Lambda=\hat{\Lambda}(\Lambda^*)^{-1}$ and check directly that $\Lambda\PP_{X^*}=\PP_{\hat{X}}\Lambda$
  and that $\nu^*\Lambda^{-1}=\hat{\nu}$. It turns out that
     $$ \Lambda(i,j)=\left\{
 \begin{array}{llll}  
  \frac{2^{j-1}(-1)^{i+j}(i-j+1){{N-1}\choose{i}}{{i}\choose{j-1}}}{(N-j)\sum_{k=0}^{i-1}{{N-1}\choose{k}}} & \mathrm{if} \ j<N, \\
  0 & j=N, i<N \\
  1 & j=N, i =N. \\
 \end{array}\right.
 $$ 
 \textcolor{red}{UWAGA: bez zastanowienia wzialem to co miales w przykladzie jako $\Lambda^{-1}$...}
 
 \textcolor{green}{ok; zmieniłem sumowanie z m na k, żeby było jak wcześniej - ale zostawiłem i (a nie m), żeby macierz była od (i,j)}
 \end{remark}


==> sections/ehrenfest2b.tex <==

Here we present a concrete example of a birth and death chain on $\E=\{1,\ldots,N\}$ with $N$ being
the only absorbing state, for which we provide $pgf$ of absorption time provided chain started at any $m\in \E$.
We use Lemma \ref{lem:duality_two_linksC} calculating link $\Lambda$. As far as we are aware, this $pgf$ 
cannot be given using results from \cite{Gong2012} \ie (\ref{eq:gTi}). 
This is since the eigenvalues the presented matrix $\PP_{X^*}$ are known, 
but the eigenvalues of $ \PP_{X^*}^{\ceil{m}}$ are not known for any $m\in\E$.
\medskip\par 

  
\begin{example}  
Let $X^*$ be a Markov Chain on the state space $ \E=\{1,\ldots, N\}$ with transition matrix ${\PP}_{X^*}$ of the form:
 $$
 {\PP}_{X^*}(i,i')=\left\{
 \begin{array}{llll}  
  \frac{N-i}{2N-2}\frac{\sum_{r=0}^{i-1} {{N-1} \choose {r-1}} }{\sum_{r=0}^{i} {{N-1} \choose {r-1}}},  & \mathrm{if }\  i'=i-1, i<N \\[12pt]
  \frac{N-2}{2N-2} & \mathrm{if} \ i'=i, i < N, \\[12pt]
  1 & \mathrm{if} \ i'=i= N, \\[12pt]
   \frac{i}{2N-2}\frac{\sum_{r=0}^{i+1} {{N-1} \choose {r-1}} }{\sum_{r=0}^{i} {{N-1} \choose {r-1}}}   & \mathrm{if }\  i'=i+1, \\[12pt]
  0 & \mathrm{otherwise}, \\
 \end{array}\right.
 $$
%and initial distribution $\nu^*(j)=\mathbb{1}_{j=m}$, e.g. $X^*$ starts in the state $m$.
Then the absorption time starting at $m\in\E $ is has the following $pgf$:
 \begin{equation}\label{eq:ex_c_pgf}
 pgf_{T_{m,d}^*}(s)=\sum_{j\leq m} \hat{\nu}(j) pgf_{\hat{T}_{j,d}}(s),
\end{equation}
where 
\begin{equation}\label{eq:hat_mu}
  \hat{\nu}(j) = \frac{2^{j-1}(-1)^{m+j}(m-j+1){{N-1}\choose{m}}{{m}\choose{j-1}}}{(N-j)\sum_{k=0}^{m-1}{{N-1}\choose{k}}}
 \quad and \quad 
 pgf_{\hat{T}_{j,N}}(s)=\prod_{k=j}^{N-1} \left[{(1-\frac{k-1}{N-1})s\over 1-\frac{k-1}{N-1} s}\right].
\end{equation}
 In particular, we have 
 \begin{equation}\label{eq:ex_c_ex}
E(T^*_{m,N})=(N-1)\sum_{j\leq m} \hat{\nu}(j) \sum_{k=j}^{N-1}{1\over N-k}.
\end{equation}

\end{example}
\begin{proof}
Let 
  $$
 {\PP}_{\hat{X}}(i,i')=\left\{
 \begin{array}{llll}  
  \frac{i-1}{N-1} & \mathrm{if} \ i'=i, \\[9pt]
  \frac{N-i}{N-1}  & \mathrm{if }\  i'=i+1, \\[9pt]
  0 & \mathrm{otherwise}. \\
 \end{array}\right.
 $$
 Note that $pgf_{\hat{T}_{j,N}}$ is obviously of form given in (\ref{eq:hat_mu}).
To show the result via Lemma \ref{lem:duality_two_linksC} it is enough 
to find $\Lambda$ such that $\Lambda \PP_{X^*}=\PP_{\hat{X}}\Lambda$ and $\nu^*\Lambda^{-1}=\hat{\nu},$
where $\nu^*(j)=\mathbbm{1}\{j=m\}$.
\par 
However, since $X^*$ has only one absorbing state, we can -- and we will -- follow the \textsl{outline of an alternative proof} 
given in Section \ref{sec:alt}. \textsl{I.e.,} we will indicate intermediate ergodic chain $X$  on $\E$ 
with transition matrix $\PP_X$ and find $\Lambda^*$ and $\hat{\Lambda}$ such that $\Lambda^*\PP_X=\PP_{X^*}\Lambda^*$
and $\hat{\Lambda}\PP_X=\PP_{\hat{X}}\hat{\Lambda}$. Then, we will automatically have 
$\Lambda=\hat{\Lambda} (\Lambda^*)^{-1}$ and we will show that $\nu^*\Lambda^{-1}=\Lambda^*(\hat{\Lambda})^{-1}=\hat{\nu}$.
\medskip\par 
\noindent
Let $X$ be a chain on $\E$ with the following transition matrix: 
$$
 {\PP}_{X}(i,i')=\left\{
 \begin{array}{llll}  
   \frac{i-1}{2(N-1)} & \mathrm{if }\  i'=i-1, \\[9pt]
  {1\over 2} & \mathrm{if} \ i'=i, \\[9pt]
  \frac{N-i}{2(N-1)}  & \mathrm{if }\  i'=i+1, \\[9pt]
  0 & \mathrm{otherwise}, \\
 \end{array}\right.
 $$
 \ie $X$ corresponds to Ehrenfest model of $N-1$ particles with an extra probability (0.5) of statying
 (and states are enumerated $1,\ldots,N$, whereas in classical Ehrenfest model these are $0,\ldots,N-1$).
 Its stationary distribution is a binomial distribution $\pi(j)={1\over 2^{N-1}}{N-1 \choose j-1}$,
 %(we have states enumerated $1,\ldots,N$ what corresponds to $0,\ldots,N-1$ in classical
 %Ehrenfest model formulation, \textcolor{green}{i.e. with probability of $\frac{1}{2}$ of staying at the present state})
  thus the classical link (cf.  (\ref{eq:link_classic})) is given by 
 $$ \Lambda^*(i,j)=\frac{{{N-1}\choose{j-1}}}{\sum_{k=0}^{i-1}{{N-1}\choose{k}}}\mathbbm{1}\{ j \leq i\},$$
 \ie we have  $\Lambda^*\PP_X=\PP_{X^*}\Lambda$ ($X^*$ is a sharp SSD of $X$). 
%  
%    It can be checked that \textcolor{red}{(pisales, ze nie jest istotna, ale to ta jest istotna, tak?) \textcolor{green}{zrobić sprawdzenie?}}
%    $$ (\Lambda^*)^{-1}(i,i')=\left\{
%  \begin{array}{llll}  
%   -\frac{\sum_{k=0}^{i-2}{{N-1}\choose{k}} }{{{N-1}\choose{i-1}}} & \mathrm{if} \ i'=i-1, \\[12pt]
%   \frac{\sum_{k=0}^{i-1}{{N-1}\choose{k}}}{{{N-1}\choose{i-1}}}  & \mathrm{if }\  i'=i, \\[10pt]
%   0 & \mathrm{otherwise}. \\
%  \end{array}\right.
%  $$
%  \par 
%  \noindent
 The eigenvalues of (Ehrenfest chain) $X$ are known, these are ${i\over N-1}, i=0,\ldots,N-1$,
 thus $\hat{X}$ is its pure birth spectral dual. The link $\hat{\Lambda}$ such that  $\hat{\Lambda}\PP_X
 =\PP_{\hat{X}}\hat{\Lambda}$ is known
 (see Eq. (4.6) in \cite{Fill2009}), it is given by
 $$\hat{\Lambda}(i,j)={ {i-1\choose j-1}\over 2^{i-1}}.$$
  It can be checked that 
   $$ \hat{\Lambda}^{-1}(i,j)=(-1)^{j-i}2^{j-1}{{i-1}\choose{j-1}}.$$
Note that $i$-th row of $\hat{\Lambda}^{-1}$ corresponds to the coefficients
\footnote{The on-line encyclopedia of integer sequences: A303872, \texttt{http://oeis.org/A303872}} in expansionn of $(2x-1)^{i-1}$
%    
%   Lambda $\Lambda=\Lambda^*\hat{\Lambda}^{-1}$ :
%    $$ \Lambda(i,j)=\left\{
%  \begin{array}{llll}  
%   \frac{2^{j-1}(-1)^{i+j}(i-j+1){{d-1}\choose{i}}{{i}\choose{j-1}}}{(d-j)\sum_{m=0}^{i-1}{{d-1}\choose{m}}} & \mathrm{if} \ j<d, \\
%   0 & i=d, j<d \\
%   1 & j=d, i =d. \\
%  \end{array}\right.
%  $$
%  
 
\noindent
Thus, as outlined in Section \ref{sec:alt} we have $\Lambda \PP_{X^*}=\PP_{\hat{X}}\Lambda$ 
 with $\Lambda=\Lambda^*(\hat{\Lambda})^{-1}$ 
 %(note that we do not need to calculate it actually) \textcolor{green}{(ale jednak musimy, bo to te same obliczenia co do $\nu^*$, więc chyba można ominąć ten nawias i ostatni Remark przeformułować tak, żeby to był wniosek z obliczenia $\nu^*$)}. We need only to check that $\nu^*\Lambda^{-1}=\nu^*\hat{\Lambda}(\Lambda^*)^{-1}$
 is equal to $\hat{\nu}$ given in (\ref{eq:hat_mu}).
 We have 
 $$(\nu^*\hat{\Lambda}(\Lambda^*)^{-1})(j) = \sum_{k} \hat{\Lambda}(m,k)(\Lambda^*)^{-1}(k,j)$$
 \textcolor{red}{TO DO: pokazac, ze wychodzi to co ma wyjsc, tj. $\hat{\nu}(j)$ dane w  (\ref{eq:hat_mu})}
 \textcolor{green}{zrobiłem to wcześniej - na samym końcu notatek - dodałem dzisiaj jeszcze dwie linijki, żeby było jaśniej - można przenieść te obliczenia tutaj}
 
 Note that $pgf$ given in (\ref{eq:hat_mu}) corresponds to the distribution of $\sum_{k=j}^{N-1} Y_k$, where $Y_k$ is a geometric random variable with parameter ${k-1\over N-1}$ and $Y_1,\ldots,Y_{N-1}$ are independent.
 We have $EY_k={N-1\over N-k}$ thus (\ref{eq:ex_c_ex}) follows from (\ref{eq:ex_c_pgf}) and (\ref{eq:hat_mu}).
 
 \end{proof}
 
 \begin{remark}
  Note that we could  calculate $\Lambda=\hat{\Lambda}(\Lambda^*)^{-1}$ and check directly that $\Lambda\PP_{X^*}=\PP_{\hat{X}}\Lambda$
  and that $\nu^*\Lambda^{-1}=\hat{\nu}$. It turns out that
     $$ \Lambda(i,j)=\left\{
 \begin{array}{llll}  
  \frac{2^{j-1}(-1)^{i+j}(i-j+1){{N-1}\choose{i}}{{i}\choose{j-1}}}{(N-j)\sum_{k=0}^{i-1}{{N-1}\choose{k}}} & \mathrm{if} \ j<N, \\
  0 & j=N, i<N \\
  1 & j=N, i =N. \\
 \end{array}\right.
 $$ 
 \textcolor{red}{UWAGA: bez zastanowienia wzialem to co miales w przykladzie jako $\Lambda^{-1}$...}
 
 \textcolor{green}{ok; zmieniłem sumowanie z m na k, żeby było jak wcześniej - ale zostawiłem i (a nie m), żeby macierz była od (i,j)}
 \end{remark}


==> sections/old2.tex <==


 
\subsection{Strong stationary duality}
Let $X$ be an ergodic Markov chain as defined in Section \ref{sec:siegmund}. Assume that $\nu$ is its initial distribution.
Let $\widetilde{\E}=\{\widetilde{\e_1},\ldots,\widetilde{\e_N}\}$ be the, possibly different, state space of the absorbing Markov chain $Y$, with transition matrix ${\PP_Y}$
and initial distribution $\widetilde{\nu}$, whose unique absorbing state is denoted by $\widetilde{\e_N}$. 
An $N\times M$ matrix $\Lambda$ is called a \textsl{link} if it is a stochastic matrix satisfying $\Lambda(\widetilde{\e_N},\e)=\pi(\e)$. We say that $X^*$ is 
a \textsl{strong stationary dual} (SSD) of $X$ with link $\Lambda^*$ if
\begin{equation}\label{eq:duality}
\nu=\widetilde{\nu}\Lambda \quad \textrm{and} \quad \Lambda\PP_X=\PP_{Y}\Lambda.
\end{equation}
Diaconis and Fill  \cite{Diaconis1990a} prove that then the absorption time $\widetilde{T}$ of $Y$ is the so called \textsl{strong stationary time} for $X$.
This is a random variable $T$ such that $X_T$ has distribution $\pi$ and $T$ is independent of $X_T$. 
The main application is to studying the rate of convergence of an ergodic chain to its stationary distribution, since for such a random variable we always have $d_{TV}(\nu\PP_X^k,\pi)\leq sep(\nu\PP_X^k,\pi)\leq P(T>k)$,
where $d_{TV}$ stands for the \textsl{total variation distance}, and $sep$ stands for the \textsl{separation `distance'}. For details, see Diaconis and Fill  \cite{Diaconis1990a}.
We say that SSD is \textbf{sharp} if $\widetilde{T}$ corresponds to stochastically the smallest SST $T$, \ie we have $sep(\nu\PP_X^k,\pi)=P(\widetilde{T}>k)$,
the corresponding SST $T$ is often called \textbf{fastest strong stationary time (FSST)}.
\smallskip\par 
\textcolor{red}{PL: tutaj cos o couplingu... }
\subsection{M\"obius and stochastic monotonicity}
We have given the definitions, and possible applications, of Siegmund duality and strong stationary duality.
Note however, that we did not mention how to find corresponding duals. In this section we will present constructions of duals in
presence of some monotonicities.

\paragraph{Total ordering.} Let $\preceq:=\leq$ be a total ordering on a finite state space $\E=\{1,\ldots,M\}$.
The chain $Y$ is \textbf{stochastically monotone} w.r.t to total ordering if $\forall i_1\leq i_2 \textrm{ }\forall j\textrm{ } \PP_Y(i_2,\{j\}^\downarrow) \leq \PP_Y(i_1,\{j\}^\downarrow)$.
We have 
\begin{lem}[Siegmund \cite{Siegmund1976}]\label{lem:Siegmund_total}
Let $X$ be an ergodic Markov chain on $\E=\{1,\ldots,M\}$ with transition matrix $\PP_X$. Siegmund dual $Z$ (w.r.t. total ordering) exists if and only if
$X$ is stochastically monotone. In such a case $\PP_{Z}=\mathcal{F}(\PP'_{Z})$, where 
$$\PP'_{Z}(j,i)=\PP_X(i,\{j\}^\downarrow)-\PP_X(i+1,\{j\}^\downarrow)$$ for 
$i,j\in \E$ (we mean $\PP_X(i+1,\cdot)=0$).
\end{lem}
Since the proof is one line long, we present it. The main thing is to show that (\ref{eq:Siegmund_duality}) holds for $n=1$. We have
\begin{equation}\label{eq:sieg_total}
\begin{array}{lll}
 \PP'_{Z}(j,i)&=&\PP'_{Z}(j,\{i\}^\uparrow)-\PP'_{Z}(j,\{i+1\}^\uparrow) = \PP_X(i,\{j\}^\downarrow)-\PP_X(i+1,\{j\}^\downarrow). 
\end{array}
\end{equation}
The latter is nonnegative if and only if $X$ is stochastically monotone.
\begin{flushright}
$\square$ 
\end{flushright}
In general, there is no recipe on  how to find an SSD, i.e., a triple $\widetilde{\E}, \PP_Y, \Lambda$. For a specific link of truncated 
stationary distribution Diaconis and Fill  \cite{Diaconis1990a} give a recipe for a dual on the
same state space  $\widetilde{\E}=\E$ provided
that the time reversed chain $\trev{X}$ is stochastically monotone with respect to the total ordering.
(Recal that transition ot time reversed chains are given by $\trev{\PP}_Y(i,j)={\pi(j)\over\pi(i)}\PP_Y(j,i)$).

\begin{thm}Diaconis and Fill  \cite{Diaconis1990a}]\label{lem:ssd_linear}
Let $X$ be an ergodic Markov chain on $\E=\{1,\ldots,M\}$, linearly ordered by $\leq$,  with transition matrix $\PP_X$, having initial distribution $\nu$ and 
stationary distribution $\pi$. Assume that
\begin{enumerate}
 \item $g(i)={\nu(i)\over \pi(i)}$ is non-increasing,
 \item $\trev{X}$ is stochastically monotone.
\end{enumerate}
Then there exists an SSD $Y$ on $\widetilde{\E}=\E$ with initial distribution $\widetilde{\nu}$, transition matrix $\PP_{Y}$ with the following link
$$\Lambda(i,j)=\mathbf{1}(i\leq j){\pi(i)\over H(j)},$$
where $H(j) =\sum_{k\leq j} \pi(k)$. Moreover, the SSD is \textbf{sharp} and is uniquely determined by
$$
\begin{array}{lllll}
 \widetilde{v}(i) & = & H(i)(g(i)-g(i+1)), i\in\E\\[10pt]
 \PP_{Y}(i,j)&=&{H(j)\over H(i)} \left(\trev{\PP}_X(j,\{i\}^\downarrow)-\trev{\PP}_X(j+1,\{i\}^\downarrow)\right), i,j\in\E
\end{array}
$$
\end{thm}

\paragraph{Partial ordering.} 
Above results for total ordering were recently extended to partial orderings. It turns out, that in both cases M\"obius monotonicity is required.
For details of the monotonicity see \cite{Lorek2012d} (in constext of SSD) or \cite{Lorek2016_Siegmund_duality} (in context of Siegmund duality).
We will shorlty recall it here. 
We consider $\E=\{\e_1,\ldots,\e_M\}$ with given partial ordering $\preceq$. 

\begin{deff}\label{def:mob_mon}
The Markov chain $y$ with transition matrix $\PP_Y$  is \textbf{M\"obius monotone} w.r.t.\ the partial order $\preceq$ if 
$\displaystyle \C^{-1}\PP_Y \C\geq 0 $ (i.e., each entry is nonnegative). In terms of the 
transition probabilities, this means that 
\[\forall(\e_i, \e_j\in \E) \quad \sum_{\e\succeq \e_i} \mu(\e_i,\e)\PP_Y(\e,\{\e_j\}^\downarrow)\geq 0.\]
\end{deff}

Similarly, we say that function $f:\E\to\mathbb{R}$ is M\"obius monotone if $\sum_{\e:\e\preceq \e_i} f(\e)\mu(\e,\e_i)\geq 0$ for all $\e_i\in\E$.
For existence of Siegmund dual M\"obius monotonicity of $X$ is required:

\begin{thm}[\cite{Lorek2016_Siegmund_duality}]\label{thm:siegmund_dual}
Let $X\sim(\nu,\PP_X)$ be a Markov chain on $\E=\{\e_1,\ldots,\e_M\}$ with partial ordering $\preceq$. Assume $\e_1$ is the  unique minimal state
and $\e_M$ is the unique maximal state.
Then there exists a Siegmund dual $Z$ of $X$ on $\bar{\E}=\{\e_0\}\cup \E$ if and only if $X$ is M\"obius monotone.
The transition matrix of the dual is $\PP_{Z}=\mathcal{F}(\PP_Z')$, where 
\begin{equation}
 \begin{tabular}{lllll}
 $\PP'_{Z}(\e_j,\e_i) $ & = & $\displaystyle(\C^{-1}\PP_X \C)(\e_i,\e_j)=\sum_{\e'\succeq \e_i} \mu(\e_i,\e')\PP_X(\e', \{\e_j\}^\downarrow)$, & $\e_i,\e_j\in\E$.\\[8pt]
\end{tabular}
\end{equation}
\end{thm}

In \cite{Lorek2012d} we derived results for strong stationary dual on the same state space $\E=\widetilde{\E}$ with link of truncated stationary distribution 
(defined below in (\ref{eq:Link_partial})). In \cite{Lorek2016_Siegmund_duality}  we pointed out, that the dual from \cite{Lorek2012d} can be given in three steps involving calculating
Siegmund dual. We present here the combined version.

\begin{thm}[\cite{Lorek2012d} and  \cite{Lorek2016_Siegmund_duality}]
Let $X$ be an ergodic Markov chain on $\E=\{\e_1,\ldots,\e_M\}$, partially ordered by $\preceq$,  with transition matrix $\PP_X$, having initial distribution $\nu$ and 
stationary distribution $\pi$. Assume that
\begin{enumerate}
 \item $g(\e)={\nu(\e)\over \pi(\e)}$ is M\"obius monotone,
 \item $\trev{X}$ is M\"obius monotone.
\end{enumerate}
Then there exists an SSD $Y$ on $\widetilde{\E}=\E$ with initial distribution $\widetilde{\nu}$, transition matrix $\PP_{Y}$ with the following link
\begin{equation}\label{eq:Link_partial}
\Lambda(\e_i,\e_j)=\mathbf{1}(\e_i\leq \e_j){\pi(\e_i)\over H(\e_j)}, 
\end{equation}
where $H(\e_j) =\sum_{\e_k\preceq \e_j} \pi(\e_k)$. Moreover, the SSD is \textbf{sharp} and  is construced in three steps:
\begin{enumerate}
 \item Calculate $\trev{\PP}_X$, transition matrix of time reversed chain,
 \item Calculate Siegmund dual $Z$ of $\trev{\PP}_X$,
 \item $ \PP_{Y}= \diag(\mathbf{H})^{-1} \PP'_{Z}\diag(\mathbf{H}),$ where $\PP'_{Z}=\mathcal{F}^{-1}_{\e_0}(\PP_{Z})$ and $\mathbf{H}=\boldsymbol{\pi}\C$ with 
 $\boldsymbol{\pi}=(\pi(\e_1),\ldots,\pi(\e_M))$.
\end{enumerate}
\end{thm}
\begin{remark}
 \rm In \cite{Lorek2012d}  we did not note that the resulting SSD is sharp, it was done in \cite{LorekSzekli2016} (Remark 2.2, p. 78).
\end{remark}



\section{old: intertw}



\begin{lem}\label{lem:duality_two_linksC}
 Let   $X^*\sim(\nu^*,\PP_{X^*})$ and  $\hat X\sim(\hat \nu, \PP_{\hat{X}})$ be two absorbing Markov chains on state spaces $\E^*$
 and $\hat\E$ and
  unique absorbing states $\e_M^*$ and $\hat\e_M$ with initial distributions $\nu^*$ and $\hat{\nu}$ respectively.
  Assume that both chains are \textbf{sharp} strong stationary dual chains of 
  an ergodic  Markov chain  $X\sim(\nu,\PP_X)$ on state space $\E$ with  initial distribution $\nu$,
  with links $\Lambda^*$ and $\hat{\Lambda}$ respectively. 
  Then, the aborption times of respective chains, $T^*$ and $\hat{T}$,
  have the same distribution. Moreover, the chains are \textbf{intertwined} via  $\Lambda=\Lambda^*\hat{\Lambda}^{-1}$,
  \ie 
  \begin{equation}
   \hat{\nu}=\nu^*\Lambda, \quad \Lambda \hat{\PP} = \PP^* \Lambda
  \end{equation}
\end{lem}

\begin{proof}
 Let $T$ be the fastest strong stationary time for $X$, \ie $sep(\nu\PP_X^k,\pi)=P(T>k)$.
Since both $\hat{X}$ and $X^*$ are sharp SSD of $X$ we have that $sep(\nu\PP_X^k,\pi)=P(\hat{T}>k)$ 
and $sep(\nu\PP_X^k,\pi)=P(T^*>k)$, thus $\hat{T}\stackrel{dist}{=} T^*$.
Moreover, we have 
 $$\Lambda^*\PP_X=\PP_{X^*}\Lambda^*\quad \mathrm{and} \quad \hat{\Lambda}\PP=\PP_{\hat{X}}\hat{\Lambda}.$$

 
 From the latter equality we have $\PP=\hat{\Lambda}^{-1}\PP_{\hat{X}}\hat{\Lambda},$ plugging it to the first one 
 we have $\Lambda^*\hat{\Lambda}^{-1}\PP_{\hat{X}}\hat{\Lambda}=\PP_{X^*}\Lambda^*$. Multiplying 
 both side by $\hat{\Lambda}$ we have $\Lambda\PP_{\hat{X}}=\PP_{X^*}\Lambda$. Similarly,
 for initial distributions we have 
 $$ \nu=\nu^*\Lambda^* \quad \textrm{and} \ \quad \nu=\hat{\nu}\hat{\Lambda},$$
 \ie $\hat{\nu}=\nu^*\Lambda$ must hold.
\end{proof}
The intertwinings are depicted in Fig. \ref{fig:intertw}.




% \newpage 

\tikzstyle{branch}=[fill,shape=circle,minimum size=3pt,inner sep=0pt]


\begin{figure}
\begin{center}
%\begin{tikzpicture}[>=latex',scale=0.8,every node/.style={scale=1}]
\begin{tikzpicture}[scale=0.8,every node/.style={scale=1}]



% \filldraw[gray!20,thick,dotted, color=black, fill=gray!8] (-1,3.7) rectangle (14.5,4.3);
% \node[scale=0.8] at (0,4) (text_ciphertext) {\small \footnotesize Ciphertext};
 
% \filldraw[gray!20,thick,dotted, color=black, fill=gray!8] (-1,-1.3) rectangle (14.5,-0.7);
% \node[scale=0.8] at (6,-1) (text_plaintext) { Plaintext };
 
 
   %\node at (-2,4) (nodeY0) {0};
   \node at (-2.5,0) (nodePg) {$X^*$};
   \node at (0,4.5) (nodeP) {$X$};
   \node at (2.5,0) (nodePh) {$\hat{X}$};
      \draw [->, scale=0.4] (nodePg) -- (nodeP) node [midway, left=0.1cm] (TextNode1) {$\Lambda^*$}; 
      \draw [->, scale=0.4] (nodePh) -- (nodeP) node [midway, right=0.1cm] (TextNode2) {$\hat{\Lambda}$};
      \draw [->, scale=0.4] (nodePg) -- (nodePh); %node[font=\fontsize{8}{8}\selectfont] [midway, below] (TextNod3) {$\Lambda=\Lambda^* \hat{\Lambda}^{-1}$};
      
      \node at (0,-0.5) (nodeLambda) {$\Lambda^O=\Lambda^* \hat{\Lambda}^{-1}$};
      
\end{tikzpicture}
\end{center}\caption{Intertwining between absorbing chains $X^*$ and $\hat{X}$ via ergodic chain $X$.}
%\textcolor{green}{lepiej zrobić strzałki w jedną stronę, żeby było wiadomo w którą stronę działa konkretny link}
\end{figure}\label{fig:intertw}
%\draw [->] (nodeY1) -- (nodeY1X2) node[font=\fontsize{8}{8}\selectfont] [midway, above=0.05cm, sloped] (TextNode3) {$+x_2$};



\paragraph{Strong stationary duals.}
%\begin{itemize}
 %\item 
 %\textsl{Strong stationary dual with link of truncated stationary distribution.}
 %\smallskip 
 For an  ergodic stochastically monotone birth and death chain  $X$  on $\E=\{1,\ldots,M\}$  
 with  transitions given in (\ref{eq:PX_bd}), the SSD 
 resulting from Lemma \ref{lem:ssd_linear} has the following transitions:
 $$
 \begin{array}{llll}
  \PP_{X^*}(i,i-1)  & = & {H(i-1)\over H(i)} p'(i), \\[10pt]
  \PP_{X^*}(i,i+1)  & = & {H(i+1)\over H(i)} q'(i+1), \\[10pt]
  \PP_{X^*}(i,i)  & = & 1-(p'(i)+q'(i+1)), \\
 \end{array}
 $$
 which is again a birth and death chain (we skip details concerning initial distributions).\par
%  
%  and initial distribution .... \textcolor{red}{PL: mozna podac, nie wiem czy trzeba}\par 
%  Note that the SSD is a birth and death chain, with $M$ being the only absorbing state. \textcolor{red}{PL: czy wspominac,
%  ze da sie dojsc z kazdego stanu do $M$?}\par 
%  



\begin{lem}\label{lem:duality_two_linksB}
 Let   $X^*\sim(\nu^*,\PP_{X^*})$ and  $\hat X\sim(\hat \nu, \PP_{\hat{X}})$ be two absorbing Markov chains on state spaces $\E^*$
 and $\hat\E$ and
  unique absorbing states $\e_M^*$ and $\hat\e_M$ with initial distributions $\nu^*$ and $\hat{\nu}$ respectively.
  Assume that the chains are intertwined by some link $\Lambda$. If the link has the following property:


 Then, the aborption times of respective chains, $T^*$ and $\hat{T}$,
  have the same distribution.
\end{lem}
\begin{proof}
 

$$ P(T^*\leq t)=P(X^*(t)=\e^*_M)=\sum_{\e^*\in \E^*} P(X^*(t)=\e^*)\Lambda(\e^*,\hat{\e}_M)=$$
$$\sum_{\e^*\in \E^*} \sum_{\e'^*\in \E^*} \nu^*(\e^*) \PP_{X^*}^t(\e^*,\e'^*)\Lambda(\e'^*,\hat{\e}_M)=$$
$$ \sum_{\e^*\in \E^*} \sum_{\hat{\e}\in \hat{\E}} \nu^*(\e^*) \Lambda(\e^*,\hat{\e}) \PP_{\hat{X}}^t(\hat{\e},\hat{\e}_M)= \sum_{\hat{\e}\in \hat{\E}} \hat{\nu}(\hat{\e}) \PP_{\hat{X}}^t(\hat{\e},\hat{\e}_M)= P(\hat{X}(t)=\hat{\e}_M)=P(\hat{T}\leq t)$$

\end{proof}

\paragraph{Sample path construction.} It turns out that once $X^*$ and $\hat{X}$ are intertwined by some link $\Lambda$, we can create sample paths 
for $\hat{X}$ given $X^*$. We skip the details, consult \cite{FilLyz12}, Section 1.1.

\medskip\par 
Assume that (\ref{eq:link_matrices}) and (\ref{eq:link_nus}) hold for some $\Lambda$ whose rows sum up to 1, but some entries are negative.
We  say that chains  $X^*\sim(\nu^*,\PP_{X^*})$ and  $\hat X\sim(\hat \nu, \PP_{\hat{X}})$ are \textbf{quasi-intertwined} by a \textbf{quasi-link} $\Lambda$.
We have:
\begin{lem}
 Let   $X^*\sim(\nu^*,\PP_{X^*})$ and  $\hat X\sim(\hat \nu, \PP_{\hat{X}})$ be two absorbing Markov chains on state spaces $\E^*$
 and $\hat\E$ and
  unique absorbing states $\e_M^*$ and $\hat\e_M$ with initial distributions $\nu^*$ and $\hat{\nu}$ respectively.
  Assume that the chains are quasi-intertwined by some quasi-link $\Lambda$ having property (\ref{eq:Lambda_cond}).
   Then, the aborption times of respective chains, $T^*$ and $\hat{T}$,
  have the same distribution.
\end{lem}
\begin{proof}
 Nothing changes in equations in proof of Lemma \ref{lem:duality_two_linksB}
\end{proof}

\begin{lem}\label{crucial lema}
 Assume that stochastic matrices $\PP_{X^*}$ and $\PP_{\hat{X}}$ of respective chains $X^*$ and $\hat{X}$ are intertwined with quasi-link $\Lambda$ having property (\ref{eq:Lambda_cond}). Moreover, assume that 
 $X^*$ has initial distribution $\nu^*$. Then, absorption time of $\hat{X}$ has the following pgf:

$$\sum_{\hat{\e}\in \hat{\E}} \hat{\nu}(\hat{\e}) pgf_{\hat{T}_{\hat{\e}}}(s),$$
where  $\hat{\nu}=\nu^*\Lambda$ (can have negative entries!) and $\hat{T}_{\hat{\e}}$ is time to absorption in the chain $\hat{X}_{\hat{e}} \sim (\delta_{\hat{e}},\PP_{\hat{X}})$ for $\hat{\e} \in \hat{E}$.
\end{lem}


\begin{proof}

  
  
%%      \textcolor{green}{2. poniżej dla porządku liniowego!!}

%%$$= \sum_{\hat{\e}\in \hat{\E}} \hat{\nu}(\hat{\e}) \prod_{\hat{\e}\leq \e \in \hat{E}} \left[{(1-\lambda_{\e})u\over 1-\lambda_{\e} u}\right], $$

\end{proof}



\medskip\par 
\paragraph{Strong stationary antiduals.}
Now start with general birth and death chain $Z$ on $\E=\{1,\ldots,N\}$ with $N$ being the only absorbing state with transitions given in 
(\ref{eq:PZj}) with $q_1(1)=0$. 
%\begin{itemize}
%\item \textsl{Antidual resulting from Lemma \ref{lem:ssd_linear}} 
%\smallskip\par 
Denote its initial distribution by $\nu$.
Fix an arbitrary $\pi$, distribution on $\E$. Let, as in Lemma \ref{lem:ssd_linear}, the link will be 
defined $\Lambda(i,j)=1(i\leq j){\pi(i)\over H(j)}$. Then, from duality relation (\ref{eq:duality}) we can compute 
transition matrix $\PP_X$ and initial distribution $\nu^X$ of an antidual chain $X$ as follows:
$$\nu^X=\nu\Lambda^{-1}, \quad \PP_X=\Lambda^{-1}\PP_{Z}\Lambda.$$
We skip the details, but it turns out that $\PP_X$ (even if it is a stochastic matrix) is \textsl{not} a birth and death chain. 
We will need an antidual chain which \textsl{is} a birth and death chains. There is a construction yielding the desired chain,
it is given in  Theorem 3.1 in \cite{Fill2009}, which we rephrase here with our notation.

\begin{thm}[Theorem 3.1, \cite{Fill2009}]\label{ref:thm_link_bd}
 Let $Z$  be an absorbing birth and death chain on $\E=\{1,\ldots,N\}$, whose unique absorbing state is $N$, with transitions given in (\ref{eq:PZj}) (\ie case $q(1)=0$) starting at 1.
 Suppose that $p(i)>0, q(i)>0, i=1,\ldots,N-1$ and that $p(i-1)+q(i)<1$ for $1\leq i\leq N_j$. Then $Z$ is the classical (\ie resulting 
 from Lemma \ref{lem:ssd_linear}, and thus sharp) of some monotone ergodic birth and death chain $X$ with transition matrix $\PP$ on $\E$ starting at 1.
\end{thm}
Denote the link appearing in Theorem \ref{ref:thm_link_bd} by $\Lambda^*$, \ie we have 
\begin{equation}\label{eq:bd_antidual}
\nu^X=\nu\Lambda^*, \quad \Lambda^*\PP_X=\PP_{Z}\Lambda^*.
\end{equation}
For the actual construction of $X$ consult \cite{Fill2009}.

% 
% 
% Then, 
% \textcolor{red}{PL: nie wypisuje tutaj tych przejsc, ale kwestia jest taka, ze antydualny NIE bedzie lancuchem urodzin i smierci. Bedzie mial przejscia $P(i,j)>0, j=0,\ldots, i+1$. 
% Podobnie rozklad poczatkowy:Np. jesli $\nu^*=\boldsymbol{\delta})_k$ (z pr. jeden startuje w $k$),
% to bodajze $\nu(i)= \mathbf{1}(i\leq k){\pi(i)\over H(k)}$}
% 
% %\item \textsl{Antidual being birth and death chain ...} 
% \textcolor{red}{PL: mozna duzo dokladniej, opisuje tylko o co chodzi}.
 
%\end{itemize}
% 
% \subsection{Intertwining between two absorbing birth and death chains}
% The probabilistic proof of \ref{eq:gT1} (\ie Theorem \ref{thm:FillMatrix}) is actually like this:\par  
% Let $\PP_{Z_j'}$ be an absorbing Markov chain on $\E=\{1,\ldots,N_j\}$ with transitions given in (\ref{eq:PZj}) and with positive 
% eigenvalues $\lambda_k,k=1,\ldots, N_j$. Assume its initial distribution is $\nu'$.
% Let $X^*$ be the chain on $\E$ with transitions given in (\ref{eq:PXd}).
% \begin{itemize}
%  \item Let $X$ be an ergodic birth and  Markov chain on $\E$, whose classical (\ie resulting from Lemma \ref{lem:ssd_linear}) SDD is $\PP_{Z_j'}$ (\textcolor{red}{PL:
%  trzeba sie odniesc, ze troche wyzej o tym pisalismy)}. It means that 
%  \begin{equation}\label{eq:duality_a}
%   \nu_X=\nu'\Lambda_a \quad \textrm{and} \quad \Lambda_a \PP_{X}=\PP_{Z_j'}\Lambda_a  
%  \end{equation}
% 
%  \item For above $X$ construct pure-birth chain ${X}^*$ (see Theorem \ref{thm:FillPureDual}) with link $\hat{\Lambda}$ given in (\ref{eq:link_spectral}). We have 
%  \begin{equation}\label{eq:duality_b}
%  \nu_X={\nu}^*\hat{\Lambda} \qquad \textrm{and} \qquad \hat{\Lambda}\PP_X=\PP_{{X}^*} \hat{\Lambda}  
%  \end{equation}
% 
%  
%   
%   \item From Lemma \ref{lem:duality_two_links} we have ...\textcolor{red}{PL: hmm.. cos mi sie nie zgadza robie tutaj wprost}:
%   As for initial distributions we have $\nu'\Lambda_a ={\nu}^*\hat{\Lambda}$ what means that $\nu^*=\nu'\Lambda_a\hat{\Lambda}^-1$
%   From (\ref{eq:duality_a}) we have 
%  $$ \PP_{X}= \Lambda_a^{-1}\PP_{Z_j'}\Lambda_a  $$
%  Plugging into (\ref{eq:duality_b}) we have 
%  $$ \hat{\Lambda}\Lambda_a^{-1}\PP_{Z_j'}\Lambda_a=\PP_{{X}^*} \hat{\Lambda}  $$
%  Multiplying by $\Lambda_a^{-1}$ (from right)
%  $$ \hat{\Lambda}\Lambda_a^{-1}\PP_{Z_j'}=\PP_{{X}^*} \hat{\Lambda} \Lambda_a  $$
%  \ie together with initial distributions
%  \begin{equation}\label{eq:biglink}
%  \nu^*={\nu}'\Lambda \qquad \textrm{and} \qquad \Lambda \PP_{Z_j'}=\PP_{{X}^*} \Lambda,  
%  \end{equation}
%  where $$\Lambda = \hat{\Lambda}\Lambda_a^{-1}$$
%  \textcolor{red}{PL: trzeba to ladniej napisac, chodzi o to, ze startujac z ur. i smierci pochl. robimy pure-birth tez pochlaniajacy, 
%  i dla nich mamy te same czasy do pochl.  - trzeba spr. czy link $\Lambda = \hat{\Lambda}\Lambda_a^{-1}$ spelnia (\ref{eq:duality2b})
% } 
%   
% \end{itemize}

% 
% \subsection{Absorption time for birth and death chains}
% \textcolor{red}{PL: na razie to tutaj pisze, ale moze po prostu calosc ma sie znalezc w dowodzie}.
% \par 
% Note that we have all the tools to prove Theorem \ref{thm:FillMatrix} the way it was done in 
% \cite{Fill2009}. Again, let $Z'$ be an absorbing Markov chain on $\E=\{1,\ldots,N\}$ 
% with transition matrix  $\P_{Z'}$ given in  (\ref{eq:PZj}). Assume its eigenvalues 
% are nonnegative: $0< \lambda_1\leq \ldots \leq \lambda_{N} = 1$. 
% Denote  its initial distribution by $\nu'$, \ie we have $\nu'=\delta_1$ (\ie we start at 1 with probability 1).
% \begin{itemize}
%  \item We can find an ergodic birth and death chain $X$ with transition matrix $\PP_X$, for which 
%  $\PP_{Z'}$ is a sharp SSD, let $\Lambda^*$ be the corresponding link, consult (\ref{eq:bd_antidual}).
%  Since $\Lambda^*$ is lower-triangular, we have $\nu=\delta_1\Lambda^* = \delta_1$.
%   \item For above ergodic chain $X\sim(\delta_1,\PP_X)$, let $\hat{X}$ denote its pure birth chain 
%   with link $\hat{\Lambda}$ given in (\ref{eq:link_spectral}) and transition matrix
%   $\hat{\PP}_X$ given in  (\ref{eq:PXd}). The link $\hat{\Lambda}$ is also lower-triangular, 
%   thus $\hat{\mu}=\delta_1$.
% \end{itemize}
% Using Lemma \ref{lem:duality_two_links} completes the proof of Theorem \ref{thm:FillMatrix}.
% 


However, we will need a different SSD construction which is a 
 %\item 
 \textsl{pure birth} chain. This is possible in case when all the eigenvalues of $\PP_X$ are non-negative,
 denote them by   $0\leq \lambda_1\leq \ldots\leq \lambda_M=1$.
 Define $\hat{X}$ to be pure birth chain with transitions
 $$
 \hat{\PP}_{X}(i,i')=\left\{
 \begin{array}{llll}  
   1-\lambda_i & \textrm{if}  i'=i+1, \\
  \lambda_i & \textrm{if} \ i'=i \\
  0 & \textrm{otherwise} \\
 \end{array}\right.
 $$
 Fill \cite{Fill2009} proves then that the matrices $\Q_k$ are all stochastic, every row of $\Q_M$ equals $\pi$ and
 \begin{thm}[Fill \cite{Fill2009}]\label{thm:FillPureDual}
 Let $X$ be stochastically monotone, ergodic birth and death chain on $\{1,\ldots,M\}$. Then, above $\hat{X}$ with transition matrix $\hat{\PP}_{X}$ is 
 a sharp strong stationary dual of $X$ w.r.t link $\hat{\Lambda}$.  
 \end{thm}
 %\textcolor{red}{PL: de facto ten ssd jest ''optymalny``/''sharp`` (tak samo pozostale tuaj), nie wiem czy trzeba wspominac}
 %\medskip\par 
 %\end{itemize}

\section{old proof of main thm. abs. time}


 
 
 
 
 $$\bigotimes_{j\leq d} \Lambda_j   \sum_{k=1}^m b_k\left(\bigotimes_{j\leq d} \R_{X_j^{*(k)}}\right)  $$
 

 $$\PP_{X^*}  =\sum_{k=1}^m b_k\left(\bigotimes_{j\leq d} \R_{X_j^{*(k)}}\right) $$
 ddd
 $$ \PP_{\hat{X}} \Lambda $$
 rrr
$$ =\sum_{k=1}^m b_k \bigotimes_{j\leq d} \Lambda^*_j \bigotimes_{j\leq d} \hat{\Lambda}_j \left(\bigotimes_{j\leq d} \R_{\hat{X}_j^{(k)}}\right)=\Lambda\PP_{\hat{X}} $$

 
 
 
 
 
 
 
 
 


\par

Consider $d$ birth and death chains $X^*_j, j=1,\ldots,d$ on respective state spaces  $\E_j=\{1,\ldots,N_j\}$ with initial distributions $\nu^*_j$.
Denote transitions of $X^*_j$ by
\begin{equation}\label{eq:PZjj} 
 \displaystyle \PP_{X^*_j}(i,i')= \left\{ 
 \begin{array}{llllllll}
  p_j(i) & \textrm{if} & i'=i+1, \\[3pt]
  q_j(i) & \textrm{if} & i'=i-1,  \\[3pt]
  1-(p_j(i)+q_j(i))& \textrm{if} & i'=i,\\[3pt]
 \end{array}
 \right.
\end{equation}
where $q_j(N_j)=p_j(N_j)=q_j(1)=0, q_j(i)>0, i=2,\ldots, N_j-1$ and $p_j(i)>0, i=1,\ldots, N_j-1$. (\textcolor{green}{jest coś takiego jak $p_j(N_j),q_j(1)$ przecież one są poza macierzą!})
Let $X_j$  be an ergodic Markov chain on $\E_j$ with initial distribution $\nu_j$, whose
$X^*_j$ is the classical SSD, \ie the one from Theorem \ref{ref:thm_link_bd} with 
link  $\Lambda^*_j$ given in (\ref{eq:bd_antidual}). We have 
$$\Lambda^*_j \PP_{X_j}=\PP_{X^*_j}\Lambda^*_j,$$
$$\nu_j=\nu_j^* \Lambda^*_j.$$
\par
Assumption $p_j(i-1)+q_j(i)\leq 1$ for $i=1,\ldots,N_j$ implies that 
the eigenvalues of $X^*_j$ are non-negative
\begin{equation}\label{eigenval} 
0<\lambda_1^{(j)}\leq \lambda_{N_j}^{(j)}=1,
\end{equation} 
 which are also the eigenvalues of $X_j$ (because of duality relation).

\par 

Define $\hat{X}_j$ to be a pure birth chain on $\E_j$ with 
transitions
\begin{equation}\label{eq:PXhat} 
 \displaystyle \PP_{\hat{X_j}}(i,i')= \left\{ 
 \begin{array}{llllllll}
  1-\lambda_i^{(j)} & \textrm{if} \   i'=i+1, \\[3pt]
   \lambda_i^{(j)} & \textrm{if} \ i'=i,  \\[3pt]
  0 & \textrm{otherwise}.\\[3pt]
 \end{array}
 \right.
\end{equation}
From Theorem \ref{thm:FillPureDual} $\hat{X}_j$ is a sharp SSD of $X_j$, denote the link given in (\ref{eq:link_spectral}) by $\hat{\Lambda}_j$.
Denote its initial distribution by $\hat{\nu}_j$. We have 
$$\hat{\Lambda}_j \PP_{X_j}=\PP_{\hat{X}_j} \hat{\Lambda}_j,$$
$$\nu_j=\hat{\nu}_j \hat{\Lambda}_j.$$
Also
$$\hat{\Lambda}_j \PP_{X_j}=\PP_{\hat{X}_j} \hat{\Lambda}_j,$$

%In light of Lemma \ref{lem:duality_two_links}, $X^*_j$ and $\hat{X}_j$ are intertwined by link $\Lambda_j=\Lambda^*_j\hat{\Lambda}_j^{-1}$, \ie we have 
%$$\Lambda_j \PP_{\hat{X}_j}=\PP_{X^*_j}\Lambda_j.$$
Define (\textcolor{green}{można jeszcze dodefiniować Lambda j jeżeli tak jest bardziej przejrzyście})
$$\Lambda^*=\bigotimes_{j\leq d} \Lambda^*_j \hspace{3cm }\hat{\Lambda}=\bigotimes_{j\leq d} \hat{\Lambda}_j \hspace{3cm } \Lambda=\Lambda^*\hat{\Lambda}^{-1}$$

Each of the $\Lambda^*_j$ and $\hat{\Lambda}_j$ are lower-triangular and have stationary distribution $\pi_j$ in the last row. Thus last rows of lower-triangular $\Lambda^*$ and $\hat{\Lambda}$ are $\bigotimes_{j\leq d} \pi_j$ and link $\Lambda$ have a property (\ref{eq:Lambda_cond}).

\medskip

Now we want to show that $\PP_{\hat{X}}$ (given in 
(\ref{eq:PZ_general2})) and $\PP_{X^*}$ are intertwined with link $\Lambda$.

%Now, we want to find $\hat{X}$ with transition matrix $\hat{\PP}$ which is intertwined with $\PP_{Z}$ given in 
%(\ref{eq:PZ_general2}) via link $\boldsymbol{\Lambda}$. 
We thus calculate 
$$\PP_{X^*}\Lambda =\sum_{k=1}^m b_k\left(\bigotimes_{j\leq d} \R_{X_j^{*(k)}}\right)\bigotimes_{j\leq d} \Lambda^*_j \bigotimes_{j\leq d} \hat{\Lambda}_j $$
$$ =\sum_{k=1}^m b_k \bigotimes_{j\leq d} \Lambda^*_j \bigotimes_{j\leq d} \hat{\Lambda}_j \left(\bigotimes_{j\leq d} \R_{\hat{X}_j^{(k)}}\right)=\Lambda\PP_{\hat{X}} $$

where  
\begin{equation}
 \R_{\hat{X}_j^{(k)}} = 
 \left\{ 
 \begin{array}{lll}
   \PP_{\hat{X}_j}  & \mathrm{if\ } j\in A_k,\\[10pt]
  \I_j & \mathrm{if\ } j\notin A_k.\\  
 \end{array}\right.
\end{equation}
%The transitions of  weighted  products of $\hat{\PP}_j^{(k)}$ are given in (\ref{eq:abs_time_res_prod}). 
%The initial distribution of $Z$ is given by $\nu=\delta_{(1,\ldots,1)}$, from Lemma \ref{lem:duality_two_links} the initial distribution of $\hat{X}$
%is given by $\hat{\nu}=\nu\boldsymbol{\Lambda}$, and since $\boldsymbol{\Lambda}$ is a product of lower-triangle matrices, we have that 
%$\hat{\nu}=\nu=\delta_{(1,\ldots,1)}$ what completes the proof.

%\ref{thm:FillMatrix}.

Now \ref{crucial lema} completes the proof of the form pgf: 
$$ pgf_{T^*}(s)=\sum_{\hat{\e}\in \hat{\E}} \hat{\nu}(\hat{\e}) pgf_{\hat{T}_{\hat{\e}}}(s),$$
where  $\hat{\nu}=\nu^*\Lambda$ (\textcolor{green}{tutaj też?!} can have negative entries!) and $\hat{T}_{\hat{\e}}$ is time to absorption in the chain $\hat{X}_{\hat{e}} \sim (\delta_{\hat{e}},\PP_{\hat{X}})$ for $\hat{\e} \in \hat{E}$.

\medskip\par

From \ref{prop:eigen} and \ref{eigenval} we have that eigenvalues of $\PP_{X^*}$ are nonnegative.

\medskip\par

Finally, link $\Lambda$ is stochastic and lower-triangular so from $\hat{\nu}=\nu^*\Lambda$ we obtain stochastic order between those two.





